Highdicom: A Python library for standardized encoding of image annotations and machine learning model outputs in pathology and radiology

Machine learning is revolutionizing image-based diagnostics in pathology and radiology. ML models have shown promising results in research settings, but their lack of interoperability has been a major barrier for clinical integration and evaluation. The DICOM a standard specifies Information Object Definitions and Services for the representation and communication of digital images and related information, including image-derived annotations and analysis results. However, the complexity of the standard represents an obstacle for its adoption in the ML community and creates a need for software libraries and tools that simplify working with data sets in DICOM format. Here we present the highdicom library, which provides a high-level application programming interface for the Python programming language that abstracts low-level details of the standard and enables encoding and decoding of image-derived information in DICOM format in a few lines of Python code. The highdicom library ties into the extensive Python ecosystem for image processing and machine learning. Simultaneously, by simplifying creation and parsing of DICOM-compliant files, highdicom achieves interoperability with the medical imaging systems that hold the data used to train and run ML models, and ultimately communicate and store model outputs for clinical use. We demonstrate through experiments with slide microscopy and computed tomography imaging, that, by bridging these two ecosystems, highdicom enables developers to train and evaluate state-of-the-art ML models in pathology and radiology while remaining compliant with the DICOM standard and interoperable with clinical systems at all stages. To promote standardization of ML research and streamline the ML model development and deployment process, we made the library available free and open-source.

==> sections/figure-legends.tex <==
\begin{figure}
    \caption{%
        Characterizing machine learning models in terms of their inputs and outputs.
        \textbf{A}. Machine learning model depicted as a black box, which transforms inputs into outputs.
        \textbf{B}. Execution of a machine learning model and communication of model inputs and outputs between model and storage system.
        \textbf{C}. Input and output characteristics of image classification, object detection and image segmentation models.
    }
    \includegraphics[width=\textwidth]{figures/figure1}
\end{figure}


% Fig.s divided into parts should be labelled with a lower-case bold a, b, and so on

\subsection*{Fig. 1: Curation of standardized image data sets.}


\subsection*{Fig. 2: Annotation of images with clinical information using standard templates and content items.}
a. DICOM Structured Reporing (SR) template TID 1500 ``Measurement Report'' as well as additional included templates.
b. Content items included by each template.
% Value type NUM includes attributes for encoding of a numeric value and the corresponding unit of measurement, value type CODE includes attributes for encoding a coded categorical value based on standard medical ontologies, and value type SCOORD3D includes attributes for encoding the graphic type (either an individual point or a more complex shape such as a polygon) as well as the actual gaphic data (spatial coordinates).
% Value type IMAGE allows specifying ROIs stored as raster graphics by reference and it includes attributes for identifiers that uniquely identify the image containing the region as well as the region within the image.


\subsection*{Fig. 3: Spatial annotation of image regions of interest using standard graphic data types.}
% OHIF viewer

\subsection*{Fig. 4: Communication of images and image-derived information using standard web services.}
A. Component diagram showing applications, programs, and systems involved in exchange of medical image data for machine learning purposes as well as their interfaces and dependencies.
B. Interactions between client and server components for machine learning model training, evaluation, and prediction as well as data annotation and visualization using resources provided by DICOMweb RESTful Services.


\subsection*{Fig. 5: Development and evaluation of a machine learning model for detection and classification of lung cancer.}
% a. Diagram of a machine learning (ML) model depicted as a black box that can be characterized by its inputs and outputs.
% b. Conceptual overview of machine learning models for common computer vision tasks and their corresponding input and output requirements.
% * Classification
%   Output: categorical features, heatmap (class activation map)
% * Segmentation
%   Output: regions of interest (pixel map),
% * Object detection
%   Output: regression head: region of interest (sub-pixel resolution); classification head: categorical feature
% c. Example of a two-dimensional, tiled visible light whole slide microscopy image and a planar region of interest (ROI) spanning multiple image tiles at different image resolution levels.
% d. Example of a three-dimensional computed tomography image and a volumic ROI spanning multiple image slices.
% each region may be represented as a raster graphic in two-dimensional pixel matrix coordinate system in pixel unit or as vector graphic in three-dimensional patient or slide coordinate system in millimeter unit

% Python -> Jupyter notebook; JavaScript -> viewer example
% OHIF viewer with MRI and pathology image for Glioma case
% \subsection*{Fig. 5: Software tools for data annotation, report creation and visualization.}\label{subsec:figure5}

\subsection*{Supplementary Fig. 1: Example content items.}
DICOM attributes included by content items of SR template TID 1411 ``Volumetric ROI Measurements and Qualitative Evaluations``.
Value types of content items are highlighted in color.

\subsection*{Supplementary Fig. 2: Proposed DICOM Structured Reporting templates for computational pathology.}
% Templates for 3 test data sets.
%           6A  IHC
%           6B  Mutation prediction from H&E
%           6C  GLIOMA (WHO template) + Vasari...


==> sections/figures.tex <==
% Fig.s divided into parts should be labelled with a lower-case bold a, b, and so on

